Weak convergence of a measure-valued process for social networks

This article formalizes the problem of modeling social networks into an interacting particle system on random geometric graphs. Each vertex of the graph is associated with a geometric position in a latent space describing the unobserved affinity between the network members and characterizes the strength of the interaction between them. We endow the system with two recruitment mechanisms that depend on the positions of the particles in the latent space and one departure mechanism independent of the latent position. We characterize each spatial position by a Dirac measure and the system state by a measure-valued process which is the sum of all Dirac masses. Therefore, we investigate the large-scale behavior of the system. In particular, using a renormalization technique, we study the system's behavior when the initial number of particles goes to infinity. We thus show the weak convergence of the rescaled measure-valued process towards the solution of a deterministic integrodifferential equation. Finally, we present some Monte Carlo simulations with different parameter sets to illustrate the merit of our approach in modeling some phenomena encountered in real-world networks.

==> babelbst.tex <==
%%
%% This is file `merlin.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from merlin.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
%\ifcase\language \input{frenbst} \or \input{frenbst}
%\else \input{frenbst} \fi
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{r\'edacteurs}        \def\bbleds{r\'ed.}
\def\bbleditor{r\'edacteur}          \def\bbled{r\'ed.}
\def\bbledby{edit\'e par}
\def\bbledition{edition}        \def\bbledn{ed}
\def\bblvolume{tome}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n$^\mathrm{o}$}
\def\bblin{dans}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Rapport technique}
\def\bbltechrep{Rap. Tech.}
\def\bblmthesis{Th\`ese de ma\^itre}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1ere}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\`eme}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\`eme}
\def\bblfourth{Quatri\`eme}          \def\bblfourtho{4\`eme}
\def\bblfifth{Cinqui\`eme}            \def\bblfiftho{5\`eme}
\def\bblst{$^{\mbox{\scriptsize \`ere}}$}  
\def\bblnd{$^{\mbox{\scriptsize \`eme}}$}  
\def\bblrd{$^{\mbox{\scriptsize \`eme}}$}
\def\bblth{$^{\mbox{\scriptsize \`eme}}$}
\def\bbljan{janvier}  \def\bblfeb{f\'evrier}  \def\bblmar{mars}
\def\bblapr{avril}    \def\bblmay{mai}       \def\bbljun{juin}
\def\bbljul{juillet}     \def\bblaug{ao\^ut}    \def\bblsep{septembre}
\def\bbloct{octobre}  \def\bblnov{novembre}  \def\bbldec{d\'ecembre}
\endinput
%%
%% End of file `merlin.tex'.


